Secure Computation and Trustless Data Intermediaries in Data Spaces

This paper explores the integration of advanced cryptographic techniques for secure computation in data spaces to enable secure and trusted data sharing, which is essential for the evolving data economy. In addition, the paper examines the role of data intermediaries, as outlined in the EU Data Governance Act, in data spaces and specifically introduces the idea of trustless intermediaries that do not have access to their users' data. Therefore, we exploit the introduced secure computation methods, i.e. Secure Multi-Party Computation (MPC) and Fully Homomorphic Encryption (FHE), and discuss the security benefits. Overall, we identify and address key challenges for integration, focusing on areas such as identity management, policy enforcement, node selection, and access control, and present solutions through real-world use cases, including air traffic management, manufacturing, and secondary data use. Furthermore, through the analysis of practical applications, this work proposes a comprehensive framework for the implementation and standardization of secure computing technologies in dynamic, trustless data environments, paving the way for future research and development of a secure and interoperable data ecosystem.

==> content/annex.tex <==
\section{Background on Data Intermediaries}

\subsection{Evolution and Utility of Data Intermediaries}

Data intermediaries have historically served as brokers, aggregators, and facilitators of data transactions. Initially, their primary function was to collect data from various sources, standardize and clean it, and then provide it to organizations that could derive value from it. Examples include market research firms, financial data providers, and health information exchanges. These entities have helped organizations to access a broader range of data, enhance their analytics capabilities, and make more informed decisions.

With the growth in data volume and complexity, the functions of data intermediaries have expanded. They now offer a wide array of services, including:
\begin{itemize}
	\item \textbf{Data Anonymization and Privacy Management}: ensuring data privacy and compliance with regulations such as GDPR,
	\item \textbf{Data Quality Assurance}: implementing processes to ensure the accuracy, completeness, and reliability of data,
	\item \textbf{Data Integration and Interoperability}: facilitating seamless integration of data from disparate sources, and
	\item \textbf{Data Marketplace Services}: providing a platform where data can be bought, sold, or exchanged securely and transparently
\end{itemize}

\subsection{Data Intermediaries in the EU Data Governance Act}


The European Union’s Data Governance Act (DGA) aims to create a framework for the safe and effective sharing of data across sectors and member states. According to the DGA, data intermediaries are entities that provide data sharing services to enable data holders to make their data available to data users, while ensuring that the rights and interests of data subjects are protected.

The DGA establishes a comprehensive framework for data intermediaries, defining their roles, responsibilities, and the conditions under which they must operate to ensure trustworthy data sharing\cite{JRC133988}. Below, we detail the specific requirements outlined in the DGA for data intermediaries, particularly those categorized as Data Intermediation Service Providers (DISPs).

\begin{itemize}
	\item \textbf{Notification and Registration}: To operate legally, data intermediaries must undergo a mandatory notification procedure with the competent national authority. This procedure requires the submission of detailed information about the service, including (i) legal status and address of the main establishment within the EU, (ii) designated contact person, and (iii) description of the type of services provided. Once the competent authority confirms compliance with Articles 11 and 12 of the DGA, the intermediary can use the label "data intermediation services provider recognized in the Union" and display the related logo as shown in \cref{fig:eu_disp}.
	
	\begin{figure}
		\begin{center}
			\includegraphics[width=0.5\columnwidth]{figures/eu_disp.png}
		\end{center}
		\caption{Logo for EU Recognised Data Intermediary.}\label{fig:eu_disp}
	\end{figure}
	
	\item \textbf{Neutrality and Independence}: A critical requirement for DISPs is maintaining neutrality and independence. They must operate strictly as neutral third parties, which means they cannot aggregate, enrich, or transform data to add substantial value and they also cannot license the resulting data for use by third parties. DISPs must ensure that their data intermediation activities are structurally separated, both legally and economically, from any other services they provide. This structural separation prevents conflicts of interest and ensures that the business model of DISPs does not depend on making a direct profit from the data shared through them.
	
	\item \textbf{Transparency and Security}: DISPs are required to maintain high standards of transparency and security. This includes providing clear and comprehensive information about their data policies and practices, as well as implementing robust security measures to protect the data they manage. Additionally, the DGA mandates that any data and metadata acquired by DISPs can only be used to improve the data intermediation service itself, further ensuring that the data intermediary's role remains impartial.
	
	\item \textbf{Service Catalogue and Fair Pricing}: DISPs must maintain a comprehensive service catalogue detailing the functions and services available to customers. Moreover, the commercial terms for the provision of intermediation services should not depend on whether a potential data holder or data user is using other services offered by the same provider.
	
	\item \textbf{Legal Compliance and Data Subject Rights}: DISPs must ensure compliance with all relevant legal frameworks, including the General Data Protection Regulation (GDPR). They must facilitate the exercise of data subjects' rights, including data access, rectification, and portability. This compliance is crucial for building trust and promoting the adoption of data intermediation services.
	
\end{itemize}

Article 10 of the DGA \cite{DGA2022} specifies three broad types of data intermediation services that can be conceptualized as enablers of data spaces.

\begin{enumerate}
	\item \textbf{Intermediation Services Between Data Holders and Potential Data Users}: These services facilitate bilateral or multilateral exchanges of data. They include creating platforms or databases that enable the exchange or joint use of data, as well as establishing infrastructure for the interconnection of data holders with data users.
	\item \textbf{Intermediation Services Between Data Subjects or Individuals and Potential Data Users}: This category primarily deals with personal or non-personal data sharing, where individuals or data subjects seek to make their data available to potential users.
	\item \textbf{Data Cooperatives}: These are organizational structures constituted by data subjects, one-person undertakings, or SMEs. Data cooperatives help their members exercise their rights over their data, facilitating informed decisions, negotiating terms for data processing, and supporting collective data management and public interest goals.
\end{enumerate}

These roles illustrate the different functions that data intermediaries can perform, ranging from facilitating industrial data sharing to personal data management and collective data governance schemes.


==> content/disp.tex <==
\section{Data Intermediaries}\label{sec:disp}

The advent of big data has changed the way organizations and individuals interact with and utilize information. As data has become an invaluable asset, the need for secure, efficient, and reliable mechanisms to manage, share, and monetize this resource has grown. Data intermediaries have emerged as crucial facilitators in this landscape, bridging gaps between data providers and data consumers, ensuring compliance with regulatory frameworks, and enhancing the value extracted from data through various services. This chapter delves into the multifaceted role of data intermediaries, their evolution under the EU Data Governance Act, and their implementation within modern Data Spaces. Additionally, it explores advanced cryptographic techniques, such as Multi-Party Computation (MPC) and Fully Homomorphic Encryption (FHE), that aim to establish trustless data intermediaries.




\subsection{Conclusion}

Data intermediaries are critical in the modern data ecosystem, facilitating secure, efficient, and compliant data exchanges. The evolving regulatory landscape, particularly the EU Data Governance Act, underscores the importance of these entities in ensuring data privacy and fostering trust. As Data Spaces become more prevalent, the roles of data intermediaries will continue to expand, encompassing advanced cryptographic techniques to establish trustless environments. By maintaining comprehensive service catalogues and leveraging cutting-edge technologies like MPC and FHE, data intermediaries will remain at the forefront of the data-driven future, enabling organizations to harness the full potential of their data assets securely and efficiently.
